Evaluating Attribution Methods using White-Box LSTMs

Interpretability methods for neural networks are difficult to evaluate because we do not understand the black-box models typically used to test them. This paper proposes a framework in which interpretability methods are evaluated using manually constructed networks, which we call white-box networks, whose behavior is understood a priori. We evaluate five methods for producing attribution heatmaps by applying them to white-box LSTM classifiers for tasks based on formal languages. Although our white-box classifiers solve their tasks perfectly and transparently, we find that all five attribution methods fail to produce the expected model explanations.

==> heatmaps/counter_aaabbbb.tex <==
\textcolor[rgb]{0.8995343807254902,0.4406918021568627,0.34410686323529416}{\textbf{a}} \textcolor[rgb]{0.8995343807254902,0.4406918021568627,0.34410686323529416}{\textbf{a}} \textcolor[rgb]{0.8995343807254902,0.4406918021568627,0.34410686323529416}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{b}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{b}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> heatmaps/fsa_aaa.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} 

==> heatmaps/fsa_aaabb.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.42519897019607844,0.559058179764706,0.9460614570784314}{\textbf{b}} \textcolor[rgb]{0.42519897019607844,0.559058179764706,0.9460614570784314}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> heatmaps/fsa_aaabbb.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} 

==> heatmaps/fsa_aabbb.tex <==
\textcolor[rgb]{0.8995343807254902,0.4406918021568627,0.34410686323529416}{\textbf{a}} \textcolor[rgb]{0.8995343807254902,0.4406918021568627,0.34410686323529416}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> heatmaps/fsa_aacba.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8252938101686275,0.2957488380941176,0.2500254739333333}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.9367796132117647,0.5327495001098039,0.41809333948627453}{\textbf{b}} \textcolor[rgb]{0.7233152383764706,0.06889824263529411,0.16298850555294117}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} 

==> heatmaps/fsa_abaa.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8252938101686275,0.2957488380941176,0.2500254739333333}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.9367796132117647,0.5327495001098039,0.41809333948627453}{\textbf{a}} \textcolor[rgb]{0.7233152383764706,0.06889824263529411,0.16298850555294117}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} 

==> heatmaps/fsa_abacd.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.9473454036,0.7946955048,0.7169905058}{\textbf{a}} \textcolor[rgb]{0.9182816725843137,0.48417347218039214,0.37779392507058823}{\textbf{b}} \textcolor[rgb]{0.940878943,0.8055964028235294,0.7351665564705883}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.9616447383764706,0.7580291825411765,0.6617823791647058}{\textbf{d}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}} 

==> heatmaps/fsa_abcabd.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.753610618,0.830232851,0.960871157}{\textbf{a}} \textcolor[rgb]{0.9244088216823529,0.49858955783529413,0.38905901227058826}{\textbf{b}} \textcolor[rgb]{0.9658988981882353,0.7401418386039216,0.6370577074156862}{\textbf{c}} \textcolor[rgb]{0.9392537715176471,0.5395814885647059,0.4239002049294118}{\textbf{a}} \textcolor[rgb]{0.966922105,0.6519686451529412,0.5319971156235295}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}} 

==> heatmaps/fsa_acbada.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8714925112588235,0.8623093793176471,0.8570162640588236}{\textbf{a}} \textcolor[rgb]{0.8918168921215687,0.8519732770431372,0.829085274254902}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} 

==> heatmaps/fsa_acbcda.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8593850998705882,0.8644309674588235,0.8721105307882353}{\textbf{a}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{c}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.9691920510470589,0.705835675717647,0.5937042609803921}{\textbf{d}} \textcolor[rgb]{0.9491505082901961,0.7907852690666667,0.7108755943019608}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} 

==> heatmaps/fsa_bbbaa.tex <==
\textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.8995343807254902,0.4406918021568627,0.34410686323529416}{\textbf{a}} \textcolor[rgb]{0.8995343807254902,0.4406918021568627,0.34410686323529416}{\textbf{a}}  & \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} 

==> heatmaps/fsa_cFalse_aaa.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} 

==> heatmaps/fsa_cFalse_abaa.tex <==
\textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} 

==> heatmaps/fsa_cFalse_acbada.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{c}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{c}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{b}} \textcolor[rgb]{0.8836871397764705,0.8561077179529412,0.8402576701764708}{\textbf{a}} \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{d}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} 

==> heatmaps/fsa_caba.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.863391831290196,0.8650837958196078,0.8676338842627451}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} 

==> heatmaps/sp_aaacc.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} 

==> heatmaps/sp_aabb.tex <==
\textcolor[rgb]{0.8755573874313726,0.860242158862745,0.8514300660980393}{\textbf{a}} \textcolor[rgb]{0.8755573874313726,0.860242158862745,0.8514300660980393}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} 

==> heatmaps/sp_aacba.tex <==
\textcolor[rgb]{0.8714925112588235,0.8623093793176471,0.8570162640588236}{\textbf{a}} \textcolor[rgb]{0.8714925112588235,0.8623093793176471,0.8570162640588236}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.9604900613294117,0.6162764239411764,0.49546660049411767}{\textbf{a}} \textcolor[rgb]{0.9604900613294117,0.6162764239411764,0.49546660049411767}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} 

==> heatmaps/sp_acbbb.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.9028486703176472,0.8447956505882352,0.8119698337411765}{\textbf{b}} \textcolor[rgb]{0.9028486703176472,0.8447956505882352,0.8119698337411765}{\textbf{b}} \textcolor[rgb]{0.9028486703176472,0.8447956505882352,0.8119698337411765}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} 

==> heatmaps/sp_acbcda.tex <==
\textcolor[rgb]{0.9566532109764706,0.598033822717647,0.4773022923529412}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.9566532109764706,0.598033822717647,0.4773022923529412}{\textbf{c}} \textcolor[rgb]{0.9566532109764706,0.598033822717647,0.4773022923529412}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.966922105,0.6519686451529412,0.5319971156235295}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.9417279298235294,0.5464134770196079,0.429707070372549}{\textbf{c}} \textcolor[rgb]{0.9392537715176471,0.5395814885647059,0.4239002049294118}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.966922105,0.6519686451529412,0.5319971156235295}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.9417279298235294,0.5464134770196079,0.429707070372549}{\textbf{c}} \textcolor[rgb]{0.9392537715176471,0.5395814885647059,0.4239002049294118}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.763520395627451,0.17866744737254903,0.1933962318627451}{\textbf{a}} \textcolor[rgb]{0.9581760317411765,0.7712340904,0.6803010368117647}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.968203399,0.7208441,0.6122929913333334}{\textbf{c}} \textcolor[rgb]{0.9548534056117647,0.5916223450078432,0.4713374634901961}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.717434544917647,0.05111754842352939,0.15873660770196077}{\textbf{b}} \textcolor[rgb]{0.717434544917647,0.05111754842352939,0.15873660770196077}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} 

==> heatmaps/sp_acbd.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.8610536002941176,0.3629157635294118,0.2906281271764706}{\textbf{a}} \textcolor[rgb]{0.8610536002941176,0.3629157635294118,0.2906281271764706}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.8610536002941176,0.3629157635294118,0.2906281271764706}{\textbf{a}} \textcolor[rgb]{0.8610536002941176,0.3629157635294118,0.2906281271764706}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{c}} \textcolor[rgb]{0.9094595977529412,0.8393864797647058,0.8003313524235294}{\textbf{b}} \textcolor[rgb]{0.9094595977529412,0.8393864797647058,0.8003313524235294}{\textbf{d}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{d}} 

==> saturation_heatmaps/0.9_accb.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.9563709270509804,0.7751443261333334,0.6864159483098039}{\textbf{b}} 

==> saturation_heatmaps/1000_accb.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8836871397764705,0.8561077179529412,0.8402576701764708}{\textbf{b}} 

==> saturation_heatmaps/100_accb.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.925563423,0.8255172980705883,0.7711363078117647}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}} 

==> saturation_heatmaps/10_accb.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8057229630470588,0.2598131362588235,0.2305616574}{\textbf{b}} 

==> saturation_heatmaps/2_accb.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.9593847296274509,0.6103057604117648,0.4893818509411765}{\textbf{b}} 

==> saturation_heatmaps/6_accb.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.9244088216823529,0.49858955783529413,0.38905901227058826}{\textbf{b}} 

==> saturation_heatmaps/7_accb.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}}  & \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{c}} \textcolor[rgb]{0.9688625003647059,0.7108384838117647,0.5999005044313725}{\textbf{b}} 

==> saturation_heatmaps/m10_lrp.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m11_lrp.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m12_lrp.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m13_lrp.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m14_lrp.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} 

==> saturation_heatmaps/m4_lrp.tex <==
\textcolor[rgb]{0.7468380122117647,0.14002101948235293,0.17999609695686275}{\textbf{a}} \textcolor[rgb]{0.7291959318352941,0.08667893684705881,0.16724040340392157}{\textbf{a}} \textcolor[rgb]{0.2389484589019608,0.3123654946588235,0.7656759021764705}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m50_lrp.tex <==
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}}  & 
\textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{a}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} \textcolor[rgb]{0.8674276350862745,0.864376599772549,0.8626024620196079}{\textbf{b}} 

==> saturation_heatmaps/m5_lrp.tex <==
\textcolor[rgb]{0.7233152383764706,0.06889824263529411,0.16298850555294117}{\textbf{a}} \textcolor[rgb]{0.717434544917647,0.05111754842352939,0.15873660770196077}{\textbf{a}} \textcolor[rgb]{0.23437707945098038,0.3055417303294118,0.7596795275882353}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m6_lrp.tex <==
\textcolor[rgb]{0.7115538514588235,0.03333685421176469,0.1544847098509804}{\textbf{a}} \textcolor[rgb]{0.7115538514588235,0.03333685421176469,0.1544847098509804}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m7_lrp.tex <==
\textcolor[rgb]{0.7115538514588235,0.03333685421176469,0.1544847098509804}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m8_lrp.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 

==> saturation_heatmaps/m9_lrp.tex <==
\textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.705673158,0.01555616,0.150232812}{\textbf{a}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} \textcolor[rgb]{0.2298057,0.298717966,0.753683153}{\textbf{b}} 
